A Non-Intrusive Data-Driven Reduced Order Model for Parametrized CFD-DEM Numerical Simulations

The investigation of fluid-solid systems is very important in a lot of industrial processes. From a computational point of view, the simulation of such systems is very expensive, especially when a huge number of parametric configurations needs to be studied. In this context, we develop a non-intrusive data-driven reduced order model (ROM) built using the proper orthogonal decomposition with interpolation (PODI) method for Computational Fluid Dynamics (CFD) -- Discrete Element Method (DEM) simulations. The main novelties of the proposed approach rely in (i) the combination of ROM and FV methods, (ii) a numerical sensitivity analysis of the ROM accuracy with respect to the number of POD modes and to the cardinality of the training set and (iii) a parametric study with respect to the Stokes number. We test our ROM on the fluidized bed benchmark problem. The accuracy of the ROM is assessed against results obtained with the FOM both for Eulerian (the fluid volume fraction) and Lagrangian (position and velocity of the particles) quantities. We also discuss the efficiency of our ROM approach.

==> noncitebib.tex <==












@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}








%%%%%%%%5555 golshan
@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}
%clayton
@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}

@article{tsu,
  title={Discrete particle simulation of two-dimensional fluidized bed.},
  author={Tsuji, Y. and Kawaguchi, T. and Tanaka, T.},
  volume={77},
  journal={Powder Technol.},
  pages={79-87},
  year={1993}
}

@article{Xu,
  title={Numerical simulation of the gas-solid flow in a fluidized bed by combining discrete particle method with computational fluid dynamics.},
  author={Xu, B. H. and Yu, A. B.},
  volume={52},
  journal={Chemical Engineering Science},
  pages={2785–2809},
  year={1997}
}

@manual{multi,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C.T. and Schwarzkopf, J.D. and Sommerfeld, M. and Tsuji, Y.},
  year={2012}
}




@article{heat,
  title={CFD-DEM simulation of heat transfer in fluidized beds: Model verification, validation, and application},
  author={Wang, S. and Luo, K. and Hu, C. and Lin, J. and Fan, J.},
  journal={Chemical Engineering Science},
  volume={197},
  pages={280-295},
  year={2019}
}

@article{review,
  title={Review and Implementation of CFD-DEM Applied to Chemical Process Systems},
  author={Golshan, S. and Sotudeh-Gharebagh, R. and Zarghami, R. and Mostoufi, N. and  Blais, B. },
  journal={ Chemical Engineering Science },
  year={2020}
}


%validation




%%%%%%%%%%%%

@manual{foam,
  title={Openfoam user guide},
  author={Greenshields, C. J.},
  year={2016}
}

@manual{liggghts,
  title={https://www.cfdem.com/media/DEM/docu/Section_intro.html},
  author={Kloss, C.}
}

@manual{rans,
  title={RANS Simulations using OpenFOAM Software},
  author={Jones, D. A. and Chapuis, M. and Liefvendahl, M. and Norrison, D. and Widjaja, R.},
  year={2016}
}

@mastersthesis{fantin,
  title={CFD-DEM Coupling for Systems of Fluid and Non-Spherical Particles},
  author={Fantin, D.},
  year={2018},
  school={TU Delft}
}


@article{menter,
  title={Ten years of industrial experience with the sst turbulence model.},
  author={Menter, F. R. and Kuntz, M. and Langty, R.},
  journal={Turbulence, heat and mass transfer},
  volume={4},
  pages={625-632},
  year={2003}
}

@article{li,
  title={A computational investigation of transient heat transfer in pneumatic transport of granular particles.},
  author={Li, J. and Mason, D. J. },
  journal={Powder Technol.},
   volume={112},
  pages={273–282},
  year={2000}
}









%%%%%%%%%%%%
@article{patil,
  title={Comparison of CFD-DEM heat transfer simulations with infrared/visual measurements},
  author={Patil, A. V. and Peters, E. A. J. F. and Kuipers, J. A. M.},
  journal={Chem. Eng. J.},
  volume={277},
  pages={388–401},
  year={2015}
}

@mastersthesis{fois,
  title={CFD modeling of gas-solid fluidized beds in OpenFOAM: a comparison between the Eulerian-Eulerian and Eulerian-Lagrangian methods},
  author={Fois, L. and Fatti, V.},
  year={2021},
  school={Politecnico di Milano}
}

%Liu, T., Han, D., Wang, J., Johnson, M.R., 2012. Effects of septal deviation on the airflow characteristics: using computational fluid dynamics models. Acta Otolaryngol. 132, 290–298.




@article{tsuji,
  title={Lagrangian numerical simulation
of plug flow of cohesionless particles in a horizontal pipe},
  author={Tsuji, Y. and Tanaka, T. and Ishida, T.},
  journal={Powder Technol.},
  volume={71(3)},
  pages={239–250},
  year={1992}
}

@article{shafer,
  title={Force schemes in simulation of granular material},
  author={Shäfer, J. and Dippel, S. and Wolf, D. E.},
  journal={ J. de Phys. I France},
  volume={6(1)},
  pages={5–20},
  year={1996}
}

@article{deen,
  title={Review of discrete particle modeling of fluidized beds},
  author={Deen, N. G. and Van Sint Annaland, M. and Van der Hoef, M. A. and Kuipers, J. A. M.},
  journal={Chem. Eng. Sci.},
  volume={62},
  pages={28–44},
  year={2007}
}

@article{hertz,
  title={Über die berührung fester elastischer körper (on the contact of elastic solids.)},
  author={Hertz, H.},
  journal={J. Reine und Angew. Math},
  volume={92},
  pages={156–171},
  year={1882}
}

@article{issa,
  title={Solution of the implicitly discretized fluid flow equations by Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flowsoperator-splitting},
  author={Issa, R.I.},
  journal={J. Comput. Phys.},
  volume={62},
  pages={40–65},
  year={1986}
}

@article{macphe,
  title={Particle tracking in unstructured, arbitrary polyhedral meshes for use in CFD and molecular dynamics},
  author={Macpherson, G. B. and Nordin, N. and Weller, H. G.},
  journal={Commun. Numer. Methods Eng},
  volume={25},
  pages={263– 273},
  year={2009}
}

@article{su,
  title={Discrete element simulation of particle flow in arbitrarily complex geometries},
  author={Su, J. and Gu, Z. and Xu, X. Y.},
  journal={Chem. Eng. Sci.},
  volume={66},
  pages={6069–6088},
  year={2011}
}


@phdthesis{jasak,
  title={Error analysis and estimation for the finite volume method with applications to fluid flows},
  author={Fois, L. and Fatti, V.},
  year={1996},
  school={Imperial College}
}




@article{palacios,
  title={Proper-orthogonal decomposition of spatio-temporal patterns in fluidized beds},
  author={Cizmas, P. G. and Palacios, A. and O’Brien, T. and Syamlal, M.},
  journal={Chemical Engineering Science},
  volume={58},
  pages={4417-4427},
  year={2003}
}


@article{wallin,
  title={Data-driven model order reduction for granular media},
  author={Wallin, E. and Servin, M.},
  journal={Computational Particle Mechanics},
  volume={9},
  pages={15–28},
  year={2022}
}


@article{fani,
  title={Reduced-order discrete element method modeling},
  author={Boukouvala, F. and Gao, Y. and Muzzio, F. and Ierapetritou, M. G.},
  journal={Chemical Engineering Science},
  volume={95},
  pages={12-26},
  year={2013}Coupled CFD-DEM modeling: formulation, implementation and application to multiphase flows
}

@article{shuo,
  title={Development of a reduced-order model for large-scale {{E}}ulerian–{{L}}agrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}


@article{shuo2,
  title={POD-based identification approach for powder mixing mechanism in Eulerian–Lagrangian simulations},
  author={Li, S. and Duan, G. and Sakai, M.},
  journal={Advanced Powder Technology},
  volume={33},
  year={2022}
}

@article{mori,
  title={Development of a robust {{E}}ulerian–{{L}}agrangian model for the simulation of an industrial solid–fluid system},
  author={Mori, Y. and Sakai, M.},
  journal={Chemical Engineering Journal},
  volume={406},
  year={2021}
}





@article{hajisharifi2021particle,
  title={Particle capture by drops in turbulent flow},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Physical Review Fluids},
  volume={6},
  number={2},
  pages={024303},
  year={2021},
  publisher={APS}
}

@article{hajisharifi2022interface,
  title={Interface topology and evolution of particle patterns on deformable drops in turbulence},
  author={Hajisharifi, A. and Marchioli, C. and Soldati, A.},
  journal={Journal of Fluid Mechanics},
  volume={933},
  year={2022},
  publisher={Cambridge University Press}
}

@book{clayton,
  title={Multiphase Flows with Droplets and Particles},
  author={Crowe, C. T. and Schwarzkopf, J. D. and Sommerfeld, M. and Tsuji, Y.},
  publisher={CRC Press},
  number={2},
  year={2011}
}







%%%% cite{fernandes} already exists!
%@article{fernandes2018validation,
%  title={Validation of the CFD-DPM solver DPMFoam in $$$\backslash$hbox $\{$OpenFOAM$\}$\^{}$\backslash$circledR $$ OpenFOAM{\textregistered} through analytical, numerical and experimental comparisons},
%  author={Fernandes, C and Semyonov, D and Ferr{\'a}s, LL and N{\'o}brega, J Miguel},
%  journal={Granular Matter},
%  volume={20},
%  number={4},
%  pages={1--18},
%  year={2018},
%  publisher={Springer}
%}

@misc{macher2006pharmaceutical,
  title={Pharmaceutical Industry Wastes $50$ Billion a Year due to Inefficient Manufacturing},
  author={Macher, J. and Nickerson, J.},
  year={2006},
  publisher={McDonough School of Business, Georgetown University, Washington, DC}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ROM papers -introduction
@book{hesthaven2016certified,
  title={Certified reduced basis methods for parametrized partial differential equations},
  author={Hesthaven, J. S. and Rozza, G. and Stamm, B.},
  volume={590},
  year={2016},
  publisher={Springer}
}

@book{quarteroni2015reduced,
  title={Reduced basis methods for partial differential equations: an introduction},
  author={Quarteroni, A. and Manzoni, A. and Negri, F.},
  volume={92},
  year={2015},
  publisher={Springer}
}

@article{benner2015survey,
  title={A survey of projection-based model reduction methods for parametric dynamical systems},
  author={Benner, P. and Gugercin, S. and Willcox, K.},
  journal={SIAM review},
  volume={57},
  number={4},
  pages={483--531},
  year={2015},
  publisher={SIAM}
}

@misc{benner2017model,
  title={Model Reduction of Parametrized Systems., volume 1st ed. 2017 of MS\&A series},
  author={Benner, P. and Ohlberger, M. and Patera, A. and Rozza, G. and Urban, K.},
  year={2017},
  publisher={Springer}
}

@book{benner2021system,
  title={System-and Data-Driven Methods and Algorithms},
  author={Benner, P. and Grivet-Talocia, S. and Quarteroni, A. and Rozza, G. and Schilders, W. and Silveira, L. M. },
  year={2021},
  publisher={De Gruyter}
}


@article{bader,
  title={Certified Reduced Basis Methods for Parametrized Distributed Elliptic Optimal Control Problems with Control Constraints.},
  author={Bader, E. and Kärcher, M. and Grepl, M. A. and Veroy, K.},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  pages={A3921–A3946},
  year={2016}
}

@article{yuan2005reduced,
  title={A reduced-order model for a bubbling fluidized bed based on proper orthogonal decomposition},
  author={Yuan, T. and Cizmas, P. G. and O’Brien, T.},
  journal={Computers \& chemical engineering},
  volume={30},
  number={2},
  pages={243--259},
  year={2005},
  publisher={Elsevier}
}




%%%%%%%%%%
%POD works in industry





@article{dolci2016proper,
  title={Proper orthogonal decomposition as surrogate model for aerodynamic optimization},
  author={Dolci, V. and Arina, R.},
  journal={International Journal of Aerospace Engineering},
  volume={2016},
  year={2016},
  publisher={Hindawi}
}



@article{di2021coarse,
  title={Coarse-grain dem modelling in fluidized bed simulation: A review},
  author={Di Renzo, A. and Napolitano, E. S. and Di Maio, F.},
  journal={Processes},
  volume={9},
  number={2},
  pages={279},
  year={2021},
  publisher={MDPI}
}

%@article{piso,
%  title={Solution of the implicitly discretised fluid flow equations by operator-splitting},
%  author={Issa, R. I.},
%  journal={Journal of Computational Physics},
%   volume={62},
%  pages={40–65},
%  year={1986}
%}

